Objective-Based Hierarchical Clustering of Deep Embedding Vectors

We initiate a comprehensive experimental study of objective-based hierarchical clustering methods on massive datasets consisting of deep embedding vectors from computer vision and NLP applications. This includes a large variety of image embedding (ImageNet, ImageNetV2, NaBirds), word embedding (Twitter, Wikipedia), and sentence embedding (SST-2) vectors from several popular recent models (e.g. ResNet, ResNext, Inception V3, SBERT). Our study includes datasets with up to $4.5$ million entries with embedding dimensions up to $2048$. In order to address the challenge of scaling up hierarchical clustering to such large datasets we propose a new practical hierarchical clustering algorithm B++&C. It gives a 5%/20% improvement on average for the popular Moseley-Wang (MW) / Cohen-Addad et al. (CKMM) objectives (normalized) compared to a wide range of classic methods and recent heuristics. We also introduce a theoretical algorithm B2SAT&C which achieves a $0.74$-approximation for the CKMM objective in polynomial time. This is the first substantial improvement over the trivial $2/3$-approximation achieved by a random binary tree. Prior to this work, the best poly-time approximation of $\approx 2/3 + 0.0004$ was due to Charikar et al. (SODA'19).

==> app_results.tex <==
\begin{comment}
    \todo{Remove this section}
    \subsection{Additional transferability experiments}
    In Table~\ref{tab:transfer_same_hpo_additional} we show additional results regarding transferability of dendrogram purity, this result is an extension of Table~\ref{tab:transfer_same_hpo}. We observe a positive correlation between $\purity$ and Top-1 error, which is not straightforward since \nabirds and \imagenet ILSVRC 2012 have a small intersection in classes. As shown in~\cite{KornblithSL19transfer} there is a relationship between the performance of supervised transfer learning and the accuracy of a neural network. 
    %We show that better neural networks transfer better also from the unsupervised point of view.
    
    
    \begin{table*}[htb]
    \centering
    \caption{Results for dendrogram purity $\purity$ of trees constructed by \ouralgo on embedding vectors by various networks for the \nabirds dataset (hyperparameters chosen for best performance using ResNet34).
    }
    \label{tab:transfer_same_hpo_additional}
    \setlength{\tabcolsep}{0.2em}
    \begin{tabular}{cSSSSSSS}
    \hline
     & \multiline{resnet\\18} &\multiline{mobilenet\\v2} & \multiline{resnet\\34} & \multiline{inception\\v3} & \multiline{resnext\\50 32x4d} & \multiline{resnet\\152} & \multiline{resnext\\101 32x8d}\\
    \hline
    \multiline{Error\footnotemark} & 30.24\% & 28.12\% & 26.7\% & 22.55\% & 22.38\% & 21.69\% & 20.69\%\\
    \hline
    $\purity$ & \cellcolor[rgb]{0.92, 0.97, 0.90}$.09$ & \cellcolor[rgb]{0.91, 0.97, 0.90}$.10$ & \cellcolor[rgb]{0.91, 0.97, 0.90}$.10$ & \cellcolor[rgb]{0.92, 0.97, 0.91}$.09$ & \cellcolor[rgb]{0.89, 0.96, 0.87}$.13$ & \cellcolor[rgb]{0.90, 0.96, 0.88}$.13$ & \cellcolor[rgb]{0.88, 0.95, 0.85}$.15$\\
    \hline
    \end{tabular}
    \end{table*}
    \footnotetext{Top-1 error on \imagenet ILSVRC 2012}
\end{comment}

\begin{comment}

\section{Algorithms}
% \ghhc~\cite{MonathZSMA19ghhc} is a gradient-based algorithm that optimizes hierarchical tree in hyperbolic space; \grinch~\cite{MonathKGM19grinch} is an online tree-based approach that uses reconfigure the hierarchy after each point insertion; \perch~\cite{KobrenMKM17perch} is another online tree-based  approach that uses local rotation as a new point arrived; \birch~\cite{ZhangRL96birch} is a top-down online hierarchical clustering that builds a tree using mean and variance statistics; \hkmeans (Hierarchical K-Means) is a top-down dividing method that recursively bisects points using Lloyd’s algorithm; \hdbscan~\cite{McinnesH2017hdbscan} is a density based method; Affinity clustering~\cite{BateniBDHKLM17} is a bottom-up approach based on building of a minimal spanning tree; Hierarchical Agglomerative Clustering is a widely used class of algorithms that includes Ward's method, Average Linkage, Single Linkage and Complete Linkage; \textsc{Random} constructs a random hierarchical clustering;


\begin{itemize}[noitemsep,nolistsep,topsep=0pt,leftmargin=*]
    \item \ghhc~\cite{MonathZSMA19ghhc} is a gradient-based algorithm that optimizes hierarchical tree in hyperbolic space
    \item \grinch~\cite{MonathKGM19grinch} and \perch~\cite{KobrenMKM17perch} are online tree-based approaches that reconfigures the hierarchy after each point insertion
    \item \birch~\cite{ZhangRL96birch} is a top-down online hierarchical clustering method that builds a tree using mean and variance statistics
    \item \hkmeans (Hierarchical K-Means) is a top-down dividing method that recursively bisects points using Lloyd’s algorithm
    \item \hdbscan~\cite{McinnesH2017hdbscan} is a density based method, builds a robust single linkage tree
    \item Affinity clustering~\cite{BateniBDHKLM17} is a bottom-up single-linkage like approach
    \item Hierarchical Agglomerative Clustering is a widely used class of algorithms that includes Ward's method, Average Linkage, Single Linkage and Complete Linkage
    \item \textsc{Random} constructs a random hierarchical clustering
    \item BBisection (Balanced bisection) is \ouralgo with imbalance $\imbalance = 0$.
    \item 2SAT is an implementation of theoretical method from our work, that uses a modified loss function of gradient based balanced bisection to solve balanced 2SAT on the top level and then runs BBisection.
    \item Random cut makes random projection on 1D vector and then runs randomized 1D clustering
\end{itemize}
\end{comment}








==> bi.tex <==
\section{Broader Impacts}
Algorithms for hierarchical clustering developed in this work have a high potential for broader impacts due to:
\begin{itemize}
    \item Applicability to virtually any datasets which can be represented as high-dimensional feature vectors. This can include not just text and images but also personal records, videos, etc. Application domains of our algorithms can range from medical and biological to satellite data, making the scope very broad. As a concrete example, a potentially interesting case study could be hierarchical clustering of Google Patent Research Data\footnote{\url{https://console.cloud.google.com/marketplace/details/google_patents_public_datasets/google-patents-research-data?pli=1}}. 
    \item High demand for quality data representations from the industry (including Google, Facebook, Amazon, etc.).
    \item High relevance to modern educational curricula focused on machine learning, data science, and AI.    
\end{itemize}

==> tables/dp.tex <==
\begin{table*}[htb]
\centering

\setlength{\tabcolsep}{0.2em}
\begin{tabular}{cPPPPP}
\hline 
\MtabSetup & \MimagenetSmall & \MimagenetBig  & \MimagenetVTwo & \Mnabirds & \MsstTwo \\
\hline

\textbf{\ouralgo} & \cellcolor[rgb]{0.85, 0.94, 0.83}$.18$ & \cellcolor[rgb]{0.90, 0.96, 0.88}$.12$ & \boldmath{\cellcolor[rgb]{0.33, 0.71, 0.40}$.58$} & \boldmath{\cellcolor[rgb]{0.91, 0.96, 0.89}$.11$} & \boldmath{\cellcolor[rgb]{0.22, 0.63, 0.34}$.72$}\\
\textbf{\oursatalgo} & \cellcolor[rgb]{0.85, 0.94, 0.83}$.18$ & \cellcolor[rgb]{0.90, 0.96, 0.88}$.13$ & \boldmath{\cellcolor[rgb]{0.33, 0.71, 0.40}$.58$} & \boldmath{\cellcolor[rgb]{0.91, 0.96, 0.89}$.11$} & \cellcolor[rgb]{0.23, 0.64, 0.35}$.70$\\
\textbf{\bbisection} & \cellcolor[rgb]{0.85, 0.94, 0.83}$.18$ & \cellcolor[rgb]{0.90, 0.96, 0.88}$.12$ & \boldmath{\cellcolor[rgb]{0.33, 0.71, 0.40}$.58$} & \boldmath{\cellcolor[rgb]{0.91, 0.96, 0.89}$.11$} & \cellcolor[rgb]{0.23, 0.64, 0.35}$.70$\\
\wards & -- & -- & \cellcolor[rgb]{0.49, 0.78, 0.49}$.48$ & -- & --\\
\averageLinkage & -- & -- & \cellcolor[rgb]{0.51, 0.79, 0.51}$.46$ & -- & --\\
\grinch & \boldmath{\cellcolor[rgb]{0.83, 0.93, 0.81}$.20$} & \boldmath{\cellcolor[rgb]{0.57, 0.82, 0.56}$.42$} & \cellcolor[rgb]{0.60, 0.83, 0.58}$.40$ & \cellcolor[rgb]{0.92, 0.97, 0.91}$.08$ & \cellcolor[rgb]{0.33, 0.71, 0.40}$.57$\\
\hkmeans & \cellcolor[rgb]{0.84, 0.94, 0.81}$.19$ & \cellcolor[rgb]{0.90, 0.96, 0.89}$.11$ & \cellcolor[rgb]{0.70, 0.88, 0.68}$.32$ & \cellcolor[rgb]{0.92, 0.97, 0.91}$.08$ & \cellcolor[rgb]{0.23, 0.65, 0.35}$.69$\\
\ghhc & \boldmath{\cellcolor[rgb]{0.83, 0.93, 0.80}$.20$} & \cellcolor[rgb]{0.62, 0.85, 0.60}$.38$ & \cellcolor[rgb]{0.78, 0.91, 0.76}$.25$ & \cellcolor[rgb]{0.93, 0.97, 0.91}$.08$ & \cellcolor[rgb]{0.33, 0.71, 0.40}$.57$\\
\singleLinkage & -- & -- & \cellcolor[rgb]{0.60, 0.83, 0.58}$.40$ & -- & --\\
\affinityClustering & -- & -- & \cellcolor[rgb]{0.62, 0.84, 0.60}$.38$ & -- & --\\
\perch & \cellcolor[rgb]{0.92, 0.97, 0.90}$.09$ & \cellcolor[rgb]{0.83, 0.93, 0.80}$.20$ & \cellcolor[rgb]{0.62, 0.85, 0.60}$.38$ & \cellcolor[rgb]{0.92, 0.97, 0.91}$.08$ & \cellcolor[rgb]{0.34, 0.71, 0.41}$.57$\\
\birch & \cellcolor[rgb]{0.85, 0.94, 0.82}$.18$ & \cellcolor[rgb]{0.93, 0.97, 0.92}$.06$ & \cellcolor[rgb]{0.85, 0.94, 0.83}$.18$ & \cellcolor[rgb]{0.95, 0.98, 0.93}$.04$ & \cellcolor[rgb]{0.33, 0.71, 0.40}$.58$\\
\completeLinkage & -- & -- & \cellcolor[rgb]{0.82, 0.93, 0.79}$.21$ & -- & --\\
\hdbscan & -- & -- & \cellcolor[rgb]{0.66, 0.86, 0.63}$.36$ & \cellcolor[rgb]{0.96, 0.99, 0.95}$.01$ & \cellcolor[rgb]{0.41, 0.75, 0.44}$.52$\\
\randomCut & \cellcolor[rgb]{0.97, 0.99, 0.96}$.00$ & \cellcolor[rgb]{0.97, 0.99, 0.96}$.00$ & \cellcolor[rgb]{0.91, 0.97, 0.89}$.10$ & \cellcolor[rgb]{0.96, 0.99, 0.95}$.01$ & \cellcolor[rgb]{0.43, 0.75, 0.45}$.52$\\
\Random & \cellcolor[rgb]{0.97, 0.99, 0.96}$.00$ & \cellcolor[rgb]{0.97, 0.99, 0.96}$.00$ & \cellcolor[rgb]{0.94, 0.98, 0.93}$.05$ & \cellcolor[rgb]{0.96, 0.99, 0.95}$.01$ & \cellcolor[rgb]{0.43, 0.76, 0.45}$.51$\\


\hline
\end{tabular}
\caption{Dendrogram purity ($\purity$) for datasets with ground truth classes. \ouralgo shows best performance under ``\generalizationSetup'', ``\shiftSetup'' and ``\sentenceSetup'' settings. Among scalable algorithms \grinch and \ghhc outperform other approaches under ``\classicSetup'' setting, however their performance drops for ``\sentenceSetup''. Among non-scalable algorithms HAC methods (\wards, \averageLinkage) show competitive performance. Our theoretical algorithm \oursatalgo shows the same performance as \bbisection. See Appendix~\ref{sec:additonal_results} for full results.
%\ouralgo shows good performance (1-6\% advantage) in transfer learning, distribution shift and sentence embedding setups. On the other hand \grinch and \ghhc works very well (1-29\% advantage) for supervised learned embedding vectors.
}
\label{tab:dendrogram_purity}
\end{table*}
